Studies of $X(3872)$ and $\psi(2S)$ production in $p\bar{p}$ collisions at 1.96 TeV

We present various properties of the production of the $X(3872)$ and $\psi(2S)$ states based on 10.4 fb$^{-1}$ collected by D0 experiment in Tevatron $p \bar p$ collisions at $\sqrt{s}$ = 1.96 TeV. For both states, we measure the nonprompt fraction $f_{NP}$ of the inclusive production rate due to decays of $b$-flavored hadrons. We find the $f_{NP}$ values systematically below those obtained at the LHC. The $f_{NP}$ fraction for $\psi(2S)$ increases with transverse momentum whereas for the X(3872) it is constant within large uncertainties, in agreement with the LHC results. The ratio of prompt to nonprompt $\psi(2S)$ production, $(1 - f_{NP}) / f_{NP}$, decreases only slightly going from the Tevatron to the LHC, but for the $X(3872)$ this ratio decreases by a factor of about 3. We test the soft-pion signature of the $X(3872)$ modeled as a weakly-bound charm-meson pair by studying the production of the $X(3872)$ as a function of the kinetic energy of the $X(3872)$ and the pion in the $X(3872)\pi$ center-of-mass frame. For a subsample consistent with prompt production, the results are incompatible with a strong enhancement in the production of the $X(3872)$ at small kinetic energy of the $X(3872)$ and the $\pi$ in the $X(3872)\pi$ center-of-mass frame expected for the $X$+soft-pion production mechanism. For events consistent with being due to decays of $b$ hadrons, there is no significant evidence for the soft-pion effect but its presence at the level expected for the binding energy of 0.17 MeV and the momentum scale $\Lambda=M(\pi)$ is not ruled out.

==> author_list.tex <==
% remove these 3 lines before journal submittal.
% \centerline{author list dated 19 July 2020}
% end removal before journal submittal
%
\affiliation{LAFEX, Centro Brasileiro de Pesquisas F\'{i}sicas, Rio de Janeiro, RJ 22290, Brazil}
\affiliation{Universidade do Estado do Rio de Janeiro, Rio de Janeiro, RJ 20550, Brazil}
\affiliation{Universidade Federal do ABC, Santo Andr\'e, SP 09210, Brazil}
\affiliation{University of Science and Technology of China, Hefei 230026, People's Republic of China}
\affiliation{Universidad de los Andes, Bogot\'a, 111711, Colombia}
\affiliation{Charles University, Faculty of Mathematics and Physics, Center for Particle Physics, 116 36 Prague 1, Czech Republic}
\affiliation{Czech Technical University in Prague, 116 36 Prague 6, Czech Republic}
\affiliation{Institute of Physics, Academy of Sciences of the Czech Republic, 182 21 Prague, Czech Republic}
\affiliation{Universidad San Francisco de Quito, Quito 170157, Ecuador}
\affiliation{LPC, Universit\'e Blaise Pascal, CNRS/IN2P3, Clermont, F-63178 Aubi\`ere Cedex, France}
\affiliation{LPSC, Universit\'e Joseph Fourier Grenoble 1, CNRS/IN2P3, Institut National Polytechnique de Grenoble, F-38026 Grenoble Cedex, France}
\affiliation{CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, F-13288 Marseille Cedex 09, France}
\affiliation{LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit\'e Paris-Saclay, F-91898 Orsay Cedex, France}
\affiliation{LPNHE, Universit\'es Paris VI and VII, CNRS/IN2P3, F-75005 Paris, France}
\affiliation{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-Sur-Yvette, France}
\affiliation{IPHC, Universit\'e de Strasbourg, CNRS/IN2P3, F-67037 Strasbourg, France}
\affiliation{IPNL, Universit\'e Lyon 1, CNRS/IN2P3, F-69622 Villeurbanne Cedex, France and Universit\'e de Lyon, F-69361 Lyon CEDEX 07, France}
\affiliation{III. Physikalisches Institut A, RWTH Aachen University, 52056 Aachen, Germany}
\affiliation{Physikalisches Institut, Universit\"at Freiburg, 79085 Freiburg, Germany}
\affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, 37073 G\"ottingen, Germany}
\affiliation{Institut f\"ur Physik, Universit\"at Mainz, 55099 Mainz, Germany}
\affiliation{Ludwig-Maximilians-Universit\"at M\"unchen, 80539 M\"unchen, Germany}
\affiliation{Panjab University, Chandigarh 160014, India}
\affiliation{Delhi University, Delhi-110 007, India}
\affiliation{Tata Institute of Fundamental Research, Mumbai-400 005, India}
\affiliation{University College Dublin, Dublin 4, Ireland}
\affiliation{Korea Detector Laboratory, Korea University, Seoul, 02841, Korea}
\affiliation{CINVESTAV, Mexico City 07360, Mexico}
\affiliation{Nikhef, Science Park, 1098 XG Amsterdam, the Netherlands}
\affiliation{Radboud University Nijmegen, 6525 AJ Nijmegen, the Netherlands}
\affiliation{Joint Institute for Nuclear Research, Dubna 141980, Russia}
\affiliation{Institute for Theoretical and Experimental Physics, Moscow 117259, Russia}
\affiliation{Moscow State University, Moscow 119991, Russia}
\affiliation{Institute for High Energy Physics, Protvino, Moscow region 142281, Russia}
\affiliation{Petersburg Nuclear Physics Institute, St. Petersburg 188300, Russia}
\affiliation{Instituci\'{o} Catalana de Recerca i Estudis Avan\c{c}ats (ICREA) and Institut de F\'{i}sica d'Altes Energies (IFAE), 08193 Bellaterra (Barcelona), Spain}
\affiliation{Uppsala University, 751 05 Uppsala, Sweden}
\affiliation{Taras Shevchenko National University of Kyiv, Kiev, 01601, Ukraine}
\affiliation{Lancaster University, Lancaster LA1 4YB, United Kingdom}
\affiliation{Imperial College London, London SW7 2AZ, United Kingdom}
\affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\affiliation{University of Arizona, Tucson, Arizona 85721, USA}
\affiliation{University of California Riverside, Riverside, California 92521, USA}
\affiliation{Florida State University, Tallahassee, Florida 32306, USA}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
\affiliation{Northwestern University, Evanston, Illinois 60208, USA}
\affiliation{Indiana University, Bloomington, Indiana 47405, USA}
\affiliation{Purdue University Calumet, Hammond, Indiana 46323, USA}
\affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA}
\affiliation{Iowa State University, Ames, Iowa 50011, USA}
\affiliation{University of Kansas, Lawrence, Kansas 66045, USA}
\affiliation{Louisiana Tech University, Ruston, Louisiana 71272, USA}
\affiliation{Northeastern University, Boston, Massachusetts 02115, USA}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\affiliation{University of Mississippi, University, Mississippi 38677, USA}
\affiliation{University of Nebraska, Lincoln, Nebraska 68588, USA}
\affiliation{Rutgers University, Piscataway, New Jersey 08855, USA}
\affiliation{Princeton University, Princeton, New Jersey 08544, USA}
\affiliation{State University of New York, Buffalo, New York 14260, USA}
\affiliation{University of Rochester, Rochester, New York 14627, USA}
\affiliation{State University of New York, Stony Brook, New York 11794, USA}
\affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\affiliation{Langston University, Langston, Oklahoma 73050, USA}
\affiliation{University of Oklahoma, Norman, Oklahoma 73019, USA}
\affiliation{Oklahoma State University, Stillwater, Oklahoma 74078, USA}
\affiliation{Oregon State University, Corvallis, Oregon 97331, USA}
\affiliation{Brown University, Providence, Rhode Island 02912, USA}
\affiliation{University of Texas, Arlington, Texas 76019, USA}
\affiliation{Southern Methodist University, Dallas, Texas 75275, USA}
\affiliation{Rice University, Houston, Texas 77005, USA}
\affiliation{University of Virginia, Charlottesville, Virginia 22904, USA}
\affiliation{University of Washington, Seattle, Washington 98195, USA}
%
\author{V.M.~Abazov} \affiliation{Joint Institute for Nuclear Research, Dubna 141980, Russia}
\author{B.~Abbott} \affiliation{University of Oklahoma, Norman, Oklahoma 73019, USA}
\author{B.S.~Acharya} \affiliation{Tata Institute of Fundamental Research, Mumbai-400 005, India}
\author{M.~Adams} \affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\author{T.~Adams} \affiliation{Florida State University, Tallahassee, Florida 32306, USA}
\author{J.P.~Agnew} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{G.D.~Alexeev} \affiliation{Joint Institute for Nuclear Research, Dubna 141980, Russia}
\author{G.~Alkhazov} \affiliation{Petersburg Nuclear Physics Institute, St. Petersburg 188300, Russia}
\author{A.~Alton$^{a}$} \affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{A.~Askew} \affiliation{Florida State University, Tallahassee, Florida 32306, USA}
\author{S.~Atkins} \affiliation{Louisiana Tech University, Ruston, Louisiana 71272, USA}
\author{K.~Augsten} \affiliation{Czech Technical University in Prague, 116 36 Prague 6, Czech Republic}
\author{V.~Aushev} \affiliation{Taras Shevchenko National University of Kyiv, Kiev, 01601, Ukraine}
\author{Y.~Aushev} \affiliation{Taras Shevchenko National University of Kyiv, Kiev, 01601, Ukraine}
\author{C.~Avila} \affiliation{Universidad de los Andes, Bogot\'a, 111711, Colombia}
\author{F.~Badaud} \affiliation{LPC, Universit\'e Blaise Pascal, CNRS/IN2P3, Clermont, F-63178 Aubi\`ere Cedex, France}
\author{L.~Bagby} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{B.~Baldin} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{D.V.~Bandurin} \affiliation{University of Virginia, Charlottesville, Virginia 22904, USA}
\author{S.~Banerjee} \affiliation{Tata Institute of Fundamental Research, Mumbai-400 005, India}
\author{E.~Barberis} \affiliation{Northeastern University, Boston, Massachusetts 02115, USA}
\author{P.~Baringer} \affiliation{University of Kansas, Lawrence, Kansas 66045, USA}
\author{J.F.~Bartlett} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{U.~Bassler} \affiliation{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-Sur-Yvette, France}
\author{V.~Bazterra} \affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\author{A.~Bean} \affiliation{University of Kansas, Lawrence, Kansas 66045, USA}
\author{M.~Begalli} \affiliation{Universidade do Estado do Rio de Janeiro, Rio de Janeiro, RJ 20550, Brazil}
\author{L.~Bellantoni} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{S.B.~Beri} \affiliation{Panjab University, Chandigarh 160014, India}
\author{G.~Bernardi} \affiliation{LPNHE, Universit\'es Paris VI and VII, CNRS/IN2P3, F-75005 Paris, France}
\author{R.~Bernhard} \affiliation{Physikalisches Institut, Universit\"at Freiburg, 79085 Freiburg, Germany}
\author{I.~Bertram} \affiliation{Lancaster University, Lancaster LA1 4YB, United Kingdom}
\author{M.~Besan\c{c}on} \affiliation{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-Sur-Yvette, France}
\author{R.~Beuselinck} \affiliation{Imperial College London, London SW7 2AZ, United Kingdom}
\author{P.C.~Bhat} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{S.~Bhatia} \affiliation{University of Mississippi, University, Mississippi 38677, USA}
\author{V.~Bhatnagar} \affiliation{Panjab University, Chandigarh 160014, India}
\author{G.~Blazey} \affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
\author{S.~Blessing} \affiliation{Florida State University, Tallahassee, Florida 32306, USA}
\author{K.~Bloom} \affiliation{University of Nebraska, Lincoln, Nebraska 68588, USA}
\author{A.~Boehnlein} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{D.~Boline} \affiliation{State University of New York, Stony Brook, New York 11794, USA}
\author{E.E.~Boos} \affiliation{Moscow State University, Moscow 119991, Russia}
\author{G.~Borissov} \affiliation{Lancaster University, Lancaster LA1 4YB, United Kingdom}
\author{M.~Borysova$^{l}$} \affiliation{Taras Shevchenko National University of Kyiv, Kiev, 01601, Ukraine}
\author{A.~Brandt} \affiliation{University of Texas, Arlington, Texas 76019, USA}
\author{O.~Brandt} \affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, 37073 G\"ottingen, Germany}
\author{M.~Brochmann} \affiliation{University of Washington, Seattle, Washington 98195, USA}
\author{R.~Brock} \affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{A.~Bross} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{D.~Brown} \affiliation{LPNHE, Universit\'es Paris VI and VII, CNRS/IN2P3, F-75005 Paris, France}
\author{X.B.~Bu} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Buehler} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{V.~Buescher} \affiliation{Institut f\"ur Physik, Universit\"at Mainz, 55099 Mainz, Germany}
\author{V.~Bunichev} \affiliation{Moscow State University, Moscow 119991, Russia}
\author{S.~Burdin$^{b}$} \affiliation{Lancaster University, Lancaster LA1 4YB, United Kingdom}
\author{C.P.~Buszello} \affiliation{Uppsala University, 751 05 Uppsala, Sweden}
\author{E.~Camacho-P\'erez} \affiliation{CINVESTAV, Mexico City 07360, Mexico}
\author{B.C.K.~Casey} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{H.~Castilla-Valdez} \affiliation{CINVESTAV, Mexico City 07360, Mexico}
\author{S.~Caughron} \affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{S.~Chakrabarti} \affiliation{State University of New York, Stony Brook, New York 11794, USA}
\author{K.M.~Chan} \affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA}
\author{A.~Chandra} \affiliation{Rice University, Houston, Texas 77005, USA}
\author{E.~Chapon} \affiliation{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-Sur-Yvette, France}
\author{G.~Chen} \affiliation{University of Kansas, Lawrence, Kansas 66045, USA}
\author{S.W.~Cho} \affiliation{Korea Detector Laboratory, Korea University, Seoul, 02841, Korea}
\author{S.~Choi} \affiliation{Korea Detector Laboratory, Korea University, Seoul, 02841, Korea}
\author{B.~Choudhary} \affiliation{Delhi University, Delhi-110 007, India}
\author{S.~Cihangir$^{\ddag}$} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{D.~Claes} \affiliation{University of Nebraska, Lincoln, Nebraska 68588, USA}
\author{J.~Clutter} \affiliation{University of Kansas, Lawrence, Kansas 66045, USA}
\author{M.~Cooke$^{j}$} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{W.E.~Cooper} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Corcoran$^{\ddag}$} \affiliation{Rice University, Houston, Texas 77005, USA}
\author{F.~Couderc} \affiliation{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-Sur-Yvette, France}
\author{M.-C.~Cousinou} \affiliation{CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, F-13288 Marseille Cedex 09, France}
\author{J.~Cuth} \affiliation{Institut f\"ur Physik, Universit\"at Mainz, 55099 Mainz, Germany}
\author{D.~Cutts} \affiliation{Brown University, Providence, Rhode Island 02912, USA}
\author{A.~Das} \affiliation{Southern Methodist University, Dallas, Texas 75275, USA}
\author{G.~Davies} \affiliation{Imperial College London, London SW7 2AZ, United Kingdom}
\author{S.J.~de~Jong} \affiliation{Nikhef, Science Park, 1098 XG Amsterdam, the Netherlands} \affiliation{Radboud University Nijmegen, 6525 AJ Nijmegen, the Netherlands}
\author{E.~De~La~Cruz-Burelo} \affiliation{CINVESTAV, Mexico City 07360, Mexico}
\author{F.~D\'eliot} \affiliation{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-Sur-Yvette, France}
\author{R.~Demina} \affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{D.~Denisov} \affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{S.P.~Denisov} \affiliation{Institute for High Energy Physics, Protvino, Moscow region 142281, Russia}
\author{S.~Desai} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{C.~Deterre$^{c}$} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{K.~DeVaughan} \affiliation{University of Nebraska, Lincoln, Nebraska 68588, USA}
\author{H.T.~Diehl} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Diesburg} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{P.F.~Ding} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{A.~Dominguez} \affiliation{University of Nebraska, Lincoln, Nebraska 68588, USA}
\author{A.~Drutskoy$^{q}$} \affiliation{Institute for Theoretical and Experimental Physics, Moscow 117259, Russia}
\author{A.~Dubey} \affiliation{Delhi University, Delhi-110 007, India}
\author{L.V.~Dudko} \affiliation{Moscow State University, Moscow 119991, Russia}
\author{A.~Duperrin} \affiliation{CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, F-13288 Marseille Cedex 09, France}
\author{S.~Dutt} \affiliation{Panjab University, Chandigarh 160014, India}
\author{M.~Eads} \affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
\author{D.~Edmunds} \affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{J.~Ellison} \affiliation{University of California Riverside, Riverside, California 92521, USA}
\author{V.D.~Elvira} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{Y.~Enari} \affiliation{LPNHE, Universit\'es Paris VI and VII, CNRS/IN2P3, F-75005 Paris, France}
\author{H.~Evans} \affiliation{Indiana University, Bloomington, Indiana 47405, USA}
\author{A.~Evdokimov} \affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\author{V.N.~Evdokimov} \affiliation{Institute for High Energy Physics, Protvino, Moscow region 142281, Russia}
\author{A.~Faur\'e} \affiliation{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-Sur-Yvette, France}
\author{L.~Feng} \affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
\author{T.~Ferbel} \affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{F.~Fiedler} \affiliation{Institut f\"ur Physik, Universit\"at Mainz, 55099 Mainz, Germany}
\author{F.~Filthaut} \affiliation{Nikhef, Science Park, 1098 XG Amsterdam, the Netherlands} \affiliation{Radboud University Nijmegen, 6525 AJ Nijmegen, the Netherlands}
\author{W.~Fisher} \affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{H.E.~Fisk} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Fortner} \affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
\author{H.~Fox} \affiliation{Lancaster University, Lancaster LA1 4YB, United Kingdom}
\author{J.~Franc} \affiliation{Czech Technical University in Prague, 116 36 Prague 6, Czech Republic}
\author{S.~Fuess} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{P.H.~Garbincius} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.~Garcia-Bellido} \affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{J.A.~Garc\'{\i}a-Gonz\'alez} \affiliation{CINVESTAV, Mexico City 07360, Mexico}
\author{V.~Gavrilov} \affiliation{Institute for Theoretical and Experimental Physics, Moscow 117259, Russia}
\author{W.~Geng} \affiliation{CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, F-13288 Marseille Cedex 09, France} \affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{C.E.~Gerber} \affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\author{Y.~Gershtein} \affiliation{Rutgers University, Piscataway, New Jersey 08855, USA}
\author{G.~Ginther} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{O.~Gogota} \affiliation{Taras Shevchenko National University of Kyiv, Kiev, 01601, Ukraine}
\author{G.~Golovanov} \affiliation{Joint Institute for Nuclear Research, Dubna 141980, Russia}
\author{P.D.~Grannis} \affiliation{State University of New York, Stony Brook, New York 11794, USA}
\author{S.~Greder} \affiliation{IPHC, Universit\'e de Strasbourg, CNRS/IN2P3, F-67037 Strasbourg, France}
\author{H.~Greenlee} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{G.~Grenier} \affiliation{IPNL, Universit\'e Lyon 1, CNRS/IN2P3, F-69622 Villeurbanne Cedex, France and Universit\'e de Lyon, F-69361 Lyon CEDEX 07, France}
\author{Ph.~Gris} \affiliation{LPC, Universit\'e Blaise Pascal, CNRS/IN2P3, Clermont, F-63178 Aubi\`ere Cedex, France}
\author{J.-F.~Grivaz} \affiliation{LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit\'e Paris-Saclay, F-91898 Orsay Cedex, France}
\author{A.~Grohsjean$^{c}$} \affiliation{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-Sur-Yvette, France}
\author{S.~Gr\"unendahl} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.W.~Gr{\"u}newald} \affiliation{University College Dublin, Dublin 4, Ireland}
\author{T.~Guillemin} \affiliation{LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit\'e Paris-Saclay, F-91898 Orsay Cedex, France}
\author{G.~Gutierrez} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{P.~Gutierrez} \affiliation{University of Oklahoma, Norman, Oklahoma 73019, USA}
\author{J.~Haley} \affiliation{Oklahoma State University, Stillwater, Oklahoma 74078, USA}
\author{L.~Han} \affiliation{University of Science and Technology of China, Hefei 230026, People's Republic of China}
\author{K.~Harder} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{A.~Harel} \affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{J.M.~Hauptman} \affiliation{Iowa State University, Ames, Iowa 50011, USA}
\author{J.~Hays} \affiliation{Imperial College London, London SW7 2AZ, United Kingdom}
\author{T.~Head} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{T.~Hebbeker} \affiliation{III. Physikalisches Institut A, RWTH Aachen University, 52056 Aachen, Germany}
\author{D.~Hedin} \affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
\author{H.~Hegab} \affiliation{Oklahoma State University, Stillwater, Oklahoma 74078, USA}
\author{A.P.~Heinson} \affiliation{University of California Riverside, Riverside, California 92521, USA}
\author{U.~Heintz} \affiliation{Brown University, Providence, Rhode Island 02912, USA}
\author{C.~Hensel} \affiliation{LAFEX, Centro Brasileiro de Pesquisas F\'{i}sicas, Rio de Janeiro, RJ 22290, Brazil}
\author{I.~Heredia-De~La~Cruz$^{d}$} \affiliation{CINVESTAV, Mexico City 07360, Mexico}
\author{K.~Herner} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{G.~Hesketh$^{f}$} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{M.D.~Hildreth} \affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA}
\author{R.~Hirosky} \affiliation{University of Virginia, Charlottesville, Virginia 22904, USA}
\author{T.~Hoang} \affiliation{Florida State University, Tallahassee, Florida 32306, USA}
\author{J.D.~Hobbs} \affiliation{State University of New York, Stony Brook, New York 11794, USA}
\author{B.~Hoeneisen} \affiliation{Universidad San Francisco de Quito, Quito 170157, Ecuador}
\author{J.~Hogan} \affiliation{Rice University, Houston, Texas 77005, USA}
\author{M.~Hohlfeld} \affiliation{Institut f\"ur Physik, Universit\"at Mainz, 55099 Mainz, Germany}
\author{J.L.~Holzbauer} \affiliation{University of Mississippi, University, Mississippi 38677, USA}
\author{I.~Howley} \affiliation{University of Texas, Arlington, Texas 76019, USA}
\author{Z.~Hubacek} \affiliation{Czech Technical University in Prague, 116 36 Prague 6, Czech Republic} \affiliation{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-Sur-Yvette, France}
\author{V.~Hynek} \affiliation{Czech Technical University in Prague, 116 36 Prague 6, Czech Republic}
\author{I.~Iashvili} \affiliation{State University of New York, Buffalo, New York 14260, USA}
\author{Y.~Ilchenko} \affiliation{Southern Methodist University, Dallas, Texas 75275, USA}
\author{R.~Illingworth} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.S.~Ito} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{S.~Jabeen$^{m}$} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Jaffr\'e} \affiliation{LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit\'e Paris-Saclay, F-91898 Orsay Cedex, France}
\author{A.~Jayasinghe} \affiliation{University of Oklahoma, Norman, Oklahoma 73019, USA}
\author{M.S.~Jeong} \affiliation{Korea Detector Laboratory, Korea University, Seoul, 02841, Korea}
\author{R.~Jesik} \affiliation{Imperial College London, London SW7 2AZ, United Kingdom}
\author{P.~Jiang$^{\ddag}$} \affiliation{University of Science and Technology of China, Hefei 230026, People's Republic of China}
\author{K.~Johns} \affiliation{University of Arizona, Tucson, Arizona 85721, USA}
\author{E.~Johnson} \affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{M.~Johnson} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.~Jonckheere} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{P.~Jonsson} \affiliation{Imperial College London, London SW7 2AZ, United Kingdom}
\author{J.~Joshi} \affiliation{University of California Riverside, Riverside, California 92521, USA}
\author{A.W.~Jung$^{o}$} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.~Juste} \affiliation{Instituci\'{o} Catalana de Recerca i Estudis Avan\c{c}ats (ICREA) and Institut de F\'{i}sica d'Altes Energies (IFAE), 08193 Bellaterra (Barcelona), Spain}
\author{E.~Kajfasz} \affiliation{CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, F-13288 Marseille Cedex 09, France}
\author{D.~Karmanov} \affiliation{Moscow State University, Moscow 119991, Russia}
\author{I.~Katsanos} \affiliation{University of Nebraska, Lincoln, Nebraska 68588, USA}
\author{M.~Kaur} \affiliation{Panjab University, Chandigarh 160014, India}
\author{R.~Kehoe} \affiliation{Southern Methodist University, Dallas, Texas 75275, USA}
\author{S.~Kermiche} \affiliation{CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, F-13288 Marseille Cedex 09, France}
\author{N.~Khalatyan} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.~Khanov} \affiliation{Oklahoma State University, Stillwater, Oklahoma 74078, USA}
\author{A.~Kharchilava} \affiliation{State University of New York, Buffalo, New York 14260, USA}
\author{Y.N.~Kharzheev} \affiliation{Joint Institute for Nuclear Research, Dubna 141980, Russia}
\author{I.~Kiselevich} \affiliation{Institute for Theoretical and Experimental Physics, Moscow 117259, Russia}
\author{J.M.~Kohli} \affiliation{Panjab University, Chandigarh 160014, India}
\author{A.V.~Kozelov} \affiliation{Institute for High Energy Physics, Protvino, Moscow region 142281, Russia}
\author{J.~Kraus} \affiliation{University of Mississippi, University, Mississippi 38677, USA}
\author{A.~Kumar} \affiliation{State University of New York, Buffalo, New York 14260, USA}
\author{A.~Kupco} \affiliation{Institute of Physics, Academy of Sciences of the Czech Republic, 182 21 Prague, Czech Republic}
\author{T.~Kur\v{c}a} \affiliation{IPNL, Universit\'e Lyon 1, CNRS/IN2P3, F-69622 Villeurbanne Cedex, France and Universit\'e de Lyon, F-69361 Lyon CEDEX 07, France}
\author{V.A.~Kuzmin} \affiliation{Moscow State University, Moscow 119991, Russia}
\author{S.~Lammers} \affiliation{Indiana University, Bloomington, Indiana 47405, USA}
\author{P.~Lebrun} \affiliation{IPNL, Universit\'e Lyon 1, CNRS/IN2P3, F-69622 Villeurbanne Cedex, France and Universit\'e de Lyon, F-69361 Lyon CEDEX 07, France}
\author{H.S.~Lee} \affiliation{Korea Detector Laboratory, Korea University, Seoul, 02841, Korea}
\author{S.W.~Lee} \affiliation{Iowa State University, Ames, Iowa 50011, USA}
\author{W.M.~Lee$^{\ddag}$} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{X.~Lei} \affiliation{University of Arizona, Tucson, Arizona 85721, USA}
\author{J.~Lellouch} \affiliation{LPNHE, Universit\'es Paris VI and VII, CNRS/IN2P3, F-75005 Paris, France}
\author{D.~Li} \affiliation{LPNHE, Universit\'es Paris VI and VII, CNRS/IN2P3, F-75005 Paris, France}
\author{H.~Li} \affiliation{University of Virginia, Charlottesville, Virginia 22904, USA}
\author{L.~Li} \affiliation{University of California Riverside, Riverside, California 92521, USA}
\author{Q.Z.~Li} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{J.K.~Lim} \affiliation{Korea Detector Laboratory, Korea University, Seoul, 02841, Korea}
\author{D.~Lincoln} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{J.~Linnemann} \affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{V.V.~Lipaev$^{\ddag}$} \affiliation{Institute for High Energy Physics, Protvino, Moscow region 142281, Russia}
\author{R.~Lipton} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{H.~Liu} \affiliation{Southern Methodist University, Dallas, Texas 75275, USA}
\author{Y.~Liu} \affiliation{University of Science and Technology of China, Hefei 230026, People's Republic of China}
\author{A.~Lobodenko} \affiliation{Petersburg Nuclear Physics Institute, St. Petersburg 188300, Russia}
\author{M.~Lokajicek} \affiliation{Institute of Physics, Academy of Sciences of the Czech Republic, 182 21 Prague, Czech Republic}
\author{R.~Lopes~de~Sa} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{R.~Luna-Garcia$^{g}$} \affiliation{CINVESTAV, Mexico City 07360, Mexico}
\author{A.L.~Lyon} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.K.A.~Maciel} \affiliation{LAFEX, Centro Brasileiro de Pesquisas F\'{i}sicas, Rio de Janeiro, RJ 22290, Brazil}
\author{R.~Madar} \affiliation{Physikalisches Institut, Universit\"at Freiburg, 79085 Freiburg, Germany}
\author{R.~Maga\~na-Villalba} \affiliation{CINVESTAV, Mexico City 07360, Mexico}
\author{S.~Malik} \affiliation{University of Nebraska, Lincoln, Nebraska 68588, USA}
\author{V.L.~Malyshev} \affiliation{Joint Institute for Nuclear Research, Dubna 141980, Russia}
\author{J.~Mansour} \affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, 37073 G\"ottingen, Germany}
\author{J.~Mart\'{\i}nez-Ortega} \affiliation{CINVESTAV, Mexico City 07360, Mexico}
\author{R.~McCarthy} \affiliation{State University of New York, Stony Brook, New York 11794, USA}
\author{C.L.~McGivern} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{M.M.~Meijer} \affiliation{Nikhef, Science Park, 1098 XG Amsterdam, the Netherlands} \affiliation{Radboud University Nijmegen, 6525 AJ Nijmegen, the Netherlands}
\author{A.~Melnitchouk} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{D.~Menezes} \affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
\author{P.G.~Mercadante} \affiliation{Universidade Federal do ABC, Santo Andr\'e, SP 09210, Brazil}
\author{M.~Merkin} \affiliation{Moscow State University, Moscow 119991, Russia}
\author{A.~Meyer} \affiliation{III. Physikalisches Institut A, RWTH Aachen University, 52056 Aachen, Germany}
\author{J.~Meyer$^{i}$} \affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, 37073 G\"ottingen, Germany}
\author{F.~Miconi} \affiliation{IPHC, Universit\'e de Strasbourg, CNRS/IN2P3, F-67037 Strasbourg, France}
\author{N.K.~Mondal} \affiliation{Tata Institute of Fundamental Research, Mumbai-400 005, India}
\author{M.~Mulhearn} \affiliation{University of Virginia, Charlottesville, Virginia 22904, USA}
\author{E.~Nagy} \affiliation{CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, F-13288 Marseille Cedex 09, France}
\author{M.~Narain} \affiliation{Brown University, Providence, Rhode Island 02912, USA}
\author{R.~Nayyar} \affiliation{University of Arizona, Tucson, Arizona 85721, USA}
\author{H.A.~Neal$^{\ddag}$} \affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{J.P.~Negret} \affiliation{Universidad de los Andes, Bogot\'a, 111711, Colombia}
\author{P.~Neustroev} \affiliation{Petersburg Nuclear Physics Institute, St. Petersburg 188300, Russia}
\author{H.T.~Nguyen} \affiliation{University of Virginia, Charlottesville, Virginia 22904, USA}
\author{T.~Nunnemann} \affiliation{Ludwig-Maximilians-Universit\"at M\"unchen, 80539 M\"unchen, Germany}
\author{J.~Orduna} \affiliation{Brown University, Providence, Rhode Island 02912, USA}
\author{N.~Osman} \affiliation{CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, F-13288 Marseille Cedex 09, France}
\author{A.~Pal} \affiliation{University of Texas, Arlington, Texas 76019, USA}
\author{N.~Parashar} \affiliation{Purdue University Calumet, Hammond, Indiana 46323, USA}
\author{V.~Parihar} \affiliation{Brown University, Providence, Rhode Island 02912, USA}
\author{S.K.~Park} \affiliation{Korea Detector Laboratory, Korea University, Seoul, 02841, Korea}
\author{R.~Partridge$^{e}$} \affiliation{Brown University, Providence, Rhode Island 02912, USA}
\author{N.~Parua} \affiliation{Indiana University, Bloomington, Indiana 47405, USA}
\author{A.~Patwa$^{j}$} \affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{B.~Penning} \affiliation{Imperial College London, London SW7 2AZ, United Kingdom}
\author{M.~Perfilov} \affiliation{Moscow State University, Moscow 119991, Russia}
\author{Y.~Peters} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{K.~Petridis} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{G.~Petrillo} \affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{P.~P\'etroff} \affiliation{LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit\'e Paris-Saclay, F-91898 Orsay Cedex, France}
\author{M.-A.~Pleier} \affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{V.M.~Podstavkov} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.V.~Popov} \affiliation{Institute for High Energy Physics, Protvino, Moscow region 142281, Russia}
\author{M.~Prewitt} \affiliation{Rice University, Houston, Texas 77005, USA}
\author{D.~Price} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{N.~Prokopenko} \affiliation{Institute for High Energy Physics, Protvino, Moscow region 142281, Russia}
\author{J.~Qian} \affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{A.~Quadt} \affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, 37073 G\"ottingen, Germany}
\author{B.~Quinn} \affiliation{University of Mississippi, University, Mississippi 38677, USA}
\author{P.N.~Ratoff} \affiliation{Lancaster University, Lancaster LA1 4YB, United Kingdom}
\author{I.~Razumov} \affiliation{Institute for High Energy Physics, Protvino, Moscow region 142281, Russia}
\author{I.~Ripp-Baudot} \affiliation{IPHC, Universit\'e de Strasbourg, CNRS/IN2P3, F-67037 Strasbourg, France}
\author{F.~Rizatdinova} \affiliation{Oklahoma State University, Stillwater, Oklahoma 74078, USA}
\author{M.~Rominsky} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{A.~Ross} \affiliation{Lancaster University, Lancaster LA1 4YB, United Kingdom}
\author{C.~Royon} \affiliation{Institute of Physics, Academy of Sciences of the Czech Republic, 182 21 Prague, Czech Republic}
\author{P.~Rubinov} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{R.~Ruchti} \affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA}
\author{G.~Sajot} \affiliation{LPSC, Universit\'e Joseph Fourier Grenoble 1, CNRS/IN2P3, Institut National Polytechnique de Grenoble, F-38026 Grenoble Cedex, France}
\author{A.~S\'anchez-Hern\'andez} \affiliation{CINVESTAV, Mexico City 07360, Mexico}
\author{M.P.~Sanders} \affiliation{Ludwig-Maximilians-Universit\"at M\"unchen, 80539 M\"unchen, Germany}
\author{A.S.~Santos$^{h}$} \affiliation{LAFEX, Centro Brasileiro de Pesquisas F\'{i}sicas, Rio de Janeiro, RJ 22290, Brazil}
\author{G.~Savage} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Savitskyi} \affiliation{Taras Shevchenko National University of Kyiv, Kiev, 01601, Ukraine}
\author{L.~Sawyer} \affiliation{Louisiana Tech University, Ruston, Louisiana 71272, USA}
\author{T.~Scanlon} \affiliation{Imperial College London, London SW7 2AZ, United Kingdom}
\author{R.D.~Schamberger} \affiliation{State University of New York, Stony Brook, New York 11794, USA}
\author{Y.~Scheglov$^{\ddag}$} \affiliation{Petersburg Nuclear Physics Institute, St. Petersburg 188300, Russia}
\author{H.~Schellman} \affiliation{Oregon State University, Corvallis, Oregon 97331, USA} \affiliation{Northwestern University, Evanston, Illinois 60208, USA}
\author{M.~Schott} \affiliation{Institut f\"ur Physik, Universit\"at Mainz, 55099 Mainz, Germany}
\author{C.~Schwanenberger$^{c}$} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{R.~Schwienhorst} \affiliation{Michigan State University, East Lansing, Michigan 48824, USA}
\author{J.~Sekaric} \affiliation{University of Kansas, Lawrence, Kansas 66045, USA}
\author{H.~Severini} \affiliation{University of Oklahoma, Norman, Oklahoma 73019, USA}
\author{E.~Shabalina} \affiliation{II. Physikalisches Institut, Georg-August-Universit\"at G\"ottingen, 37073 G\"ottingen, Germany}
\author{V.~Shary} \affiliation{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-Sur-Yvette, France}
\author{S.~Shaw} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{A.A.~Shchukin} \affiliation{Institute for High Energy Physics, Protvino, Moscow region 142281, Russia}
\author{O.~Shkola} \affiliation{Taras Shevchenko National University of Kyiv, Kiev, 01601, Ukraine}
\author{V.~Simak$^{\ddag}$} \affiliation{Czech Technical University in Prague, 116 36 Prague 6, Czech Republic}
\author{P.~Skubic} \affiliation{University of Oklahoma, Norman, Oklahoma 73019, USA}
\author{P.~Slattery} \affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{G.R.~Snow$^{\ddag}$} \affiliation{University of Nebraska, Lincoln, Nebraska 68588, USA}
\author{J.~Snow} \affiliation{Langston University, Langston, Oklahoma 73050, USA}
\author{S.~Snyder} \affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{S.~S{\"o}ldner-Rembold} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{L.~Sonnenschein} \affiliation{III. Physikalisches Institut A, RWTH Aachen University, 52056 Aachen, Germany}
\author{K.~Soustruznik} \affiliation{Charles University, Faculty of Mathematics and Physics, Center for Particle Physics, 116 36 Prague 1, Czech Republic}
\author{J.~Stark} \affiliation{LPSC, Universit\'e Joseph Fourier Grenoble 1, CNRS/IN2P3, Institut National Polytechnique de Grenoble, F-38026 Grenoble Cedex, France}
\author{N.~Stefaniuk} \affiliation{Taras Shevchenko National University of Kyiv, Kiev, 01601, Ukraine}
\author{D.A.~Stoyanova} \affiliation{Institute for High Energy Physics, Protvino, Moscow region 142281, Russia}
\author{M.~Strauss} \affiliation{University of Oklahoma, Norman, Oklahoma 73019, USA}
\author{L.~Suter} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{P.~Svoisky} \affiliation{University of Virginia, Charlottesville, Virginia 22904, USA}
\author{M.~Titov} \affiliation{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-Sur-Yvette, France}
\author{V.V.~Tokmenin} \affiliation{Joint Institute for Nuclear Research, Dubna 141980, Russia}
\author{Y.-T.~Tsai} \affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{D.~Tsybychev} \affiliation{State University of New York, Stony Brook, New York 11794, USA}
\author{B.~Tuchming} \affiliation{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-Sur-Yvette, France}
\author{C.~Tully} \affiliation{Princeton University, Princeton, New Jersey 08544, USA}
\author{L.~Uvarov} \affiliation{Petersburg Nuclear Physics Institute, St. Petersburg 188300, Russia}
\author{S.~Uvarov} \affiliation{Petersburg Nuclear Physics Institute, St. Petersburg 188300, Russia}
\author{S.~Uzunyan} \affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
\author{R.~Van~Kooten} \affiliation{Indiana University, Bloomington, Indiana 47405, USA}
\author{W.M.~van~Leeuwen} \affiliation{Nikhef, Science Park, 1098 XG Amsterdam, the Netherlands}
\author{N.~Varelas} \affiliation{University of Illinois at Chicago, Chicago, Illinois 60607, USA}
\author{E.W.~Varnes} \affiliation{University of Arizona, Tucson, Arizona 85721, USA}
\author{I.A.~Vasilyev} \affiliation{Institute for High Energy Physics, Protvino, Moscow region 142281, Russia}
\author{A.Y.~Verkheev} \affiliation{Joint Institute for Nuclear Research, Dubna 141980, Russia}
\author{L.S.~Vertogradov} \affiliation{Joint Institute for Nuclear Research, Dubna 141980, Russia}
\author{M.~Verzocchi} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{M.~Vesterinen} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{D.~Vilanova} \affiliation{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-Sur-Yvette, France}
\author{P.~Vokac} \affiliation{Czech Technical University in Prague, 116 36 Prague 6, Czech Republic}
\author{H.D.~Wahl} \affiliation{Florida State University, Tallahassee, Florida 32306, USA}
\author{C.~Wang} \affiliation{University of Science and Technology of China, Hefei 230026, People's Republic of China}
\author{M.H.L.S.~Wang} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{J.~Warchol$^{\ddag}$} \affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA}
\author{G.~Watts} \affiliation{University of Washington, Seattle, Washington 98195, USA}
\author{M.~Wayne} \affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA}
\author{J.~Weichert} \affiliation{Institut f\"ur Physik, Universit\"at Mainz, 55099 Mainz, Germany}
\author{L.~Welty-Rieger} \affiliation{Northwestern University, Evanston, Illinois 60208, USA}
\author{M.R.J.~Williams$^{n}$} \affiliation{Indiana University, Bloomington, Indiana 47405, USA}
\author{G.W.~Wilson} \affiliation{University of Kansas, Lawrence, Kansas 66045, USA}
\author{M.~Wobisch} \affiliation{Louisiana Tech University, Ruston, Louisiana 71272, USA}
\author{D.R.~Wood} \affiliation{Northeastern University, Boston, Massachusetts 02115, USA}
\author{T.R.~Wyatt} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{Y.~Xie} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{R.~Yamada} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{S.~Yang} \affiliation{University of Science and Technology of China, Hefei 230026, People's Republic of China}
\author{T.~Yasuda} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{Y.A.~Yatsunenko} \affiliation{Joint Institute for Nuclear Research, Dubna 141980, Russia}
\author{W.~Ye} \affiliation{State University of New York, Stony Brook, New York 11794, USA}
\author{Z.~Ye} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{H.~Yin} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{K.~Yip} \affiliation{Brookhaven National Laboratory, Upton, New York 11973, USA}
\author{S.W.~Youn} \affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
\author{J.M.~Yu} \affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{J.~Zennamo} \affiliation{State University of New York, Buffalo, New York 14260, USA}
\author{T.G.~Zhao} \affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\author{B.~Zhou} \affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{J.~Zhu} \affiliation{University of Michigan, Ann Arbor, Michigan 48109, USA}
\author{M.~Zielinski} \affiliation{University of Rochester, Rochester, New York 14627, USA}
\author{D.~Zieminska} \affiliation{Indiana University, Bloomington, Indiana 47405, USA}
\author{L.~Zivkovic$^{p}$} \affiliation{LPNHE, Universit\'es Paris VI and VII, CNRS/IN2P3, F-75005 Paris, France}
%
% visitor_addresses.tex                       19 July 2020
%  available symbols are:
%  $\ast, \dag, \ddag, \S, \P, $\|$, $\ast\ast$, \dag\dag, \ddag\ddag ,\#
%
\collaboration{The D0 Collaboration\footnote{with visitors from
%{alton}
$^{a}$Augustana College, Sioux Falls, SD 57197, USA,
%{burdin}
$^{b}$The University of Liverpool, Liverpool L69 3BX, UK,
%{grohsjean,deterre}
$^{c}$Deutshes Elektronen-Synchrotron (DESY), Notkestrasse 85, Germany,
%{de la cruz-burelo}
$^{d}$CONACyT, M-03940 Mexico City, Mexico,
%{partridge}
$^{e}$SLAC, Menlo Park, CA 94025, USA,
%{hesketh}
$^{f}$University College London, London WC1E 6BT, UK,
%{luna-garcia}
$^{g}$Centro de Investigacion en Computacion - IPN, CP 07738 Mexico City, Mexico,
%{santos}
$^{h}$Universidade Estadual Paulista, S\~ao Paulo, SP 01140, Brazil,
%{meyer}
$^{i}$Karlsruher Institut f\"ur Technologie (KIT) - Steinbuch Centre for Computing (SCC),
D-76128 Karlsruhe, Germany,
%{patwa}
$^{j}$Office of Science, U.S. Department of Energy, Washington, D.C. 20585, USA,
%{cooke}
%$^{k}$American Association for the Advancement of Science, Washington, D.C. 20005, USA,
%{borysova}
$^{l}$Kiev Institute for Nuclear Research (KINR), Kyiv 03680, Ukraine,
%{jabeen}
$^{m}$University of Maryland, College Park, MD 20742, USA,
%{williams}
$^{n}$European Orgnaization for Nuclear Research (CERN), CH-1211 Geneva, Switzerland,
%{Jung}
$^{o}$Purdue University, West Lafayette, IN 47907, USA,
%{Zivkovic}
$^{p}$Institute of Physics, Belgrade, Belgrade, Serbia,
and
%{Drutskoy}
$^{q}$P.N. Lebedev Physical Institute of the Russian Academy of Sciences, 119991, Moscow, Russia.
%{montgomery}
%$^{?}$Thomas Jefferson National Accelerator Facility, Newport News, VA 23606, USA,
%{falkowski}
%$^{?}$Laboratoire de Physique Theorique, F-91405 Orsay CEDEX, FR,
%{hooper,kozminski}
%$^{?}$}Visitor from Lewis University, Romeoville, IL 60446, USA.
%{weber}
%$^{?}$Universit{\"a}t Bern, CH-3012 Bern, Switzerland.
%{deceased}
%{peng, lipaev, cihangir}
$^{\ddag}$Deceased.
}} \noaffiliation
%
\vskip 0.25cm

